Interactive Learning for Identifying Relevant Tweets to Support Real-time Situational Awareness

Various domain users are increasingly leveraging real-time social media data to gain rapid situational awareness. However, due to the high noise in the deluge of data, effectively determining semantically relevant information can be difficult, further complicated by the changing definition of relevancy by each end user for different events. The majority of existing methods for short text relevance classification fail to incorporate users' knowledge into the classification process. Existing methods that incorporate interactive user feedback focus on historical datasets. Therefore, classifiers cannot be interactively retrained for specific events or user-dependent needs in real-time. This limits real-time situational awareness, as streaming data that is incorrectly classified cannot be corrected immediately, permitting the possibility for important incoming data to be incorrectly classified as well. We present a novel interactive learning framework to improve the classification process in which the user iteratively corrects the relevancy of tweets in real-time to train the classification model on-the-fly for immediate predictive improvements. We computationally evaluate our classification model adapted to learn at interactive rates. Our results show that our approach outperforms state-of-the-art machine learning models. In addition, we integrate our framework with the extended Social Media Analytics and Reporting Toolkit (SMART) 2.0 system, allowing the use of our interactive learning framework within a visual analytics system tailored for real-time situational awareness. To demonstrate our framework's effectiveness, we provide domain expert feedback from first responders who used the extended SMART 2.0 system.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> approach.tex <==
\section{Approach}
\subsection{Background: SMART}
The Social Media Analytics and Reporting Toolkit was primarily developed by researchers at Purdue University to provide situational awareness to first responders, government officials, and special interest groups. 
SMART obtains real-time publicly available geo-tagged data from Twitter and Instagram and displays them on a map.
The user is able to interactively explore the spatiotemporal characteristics and content of the data through a number of visualizations and filters.
Spatial interactions include filtering by geographical bounds, selecting posts on the map directly to view their content, and applying a heat map to view the spatial density.
In addition, the tweet time chart and theme river convey the temporal distributions of the data.

SMART's classifier visualization is arguably its most important feature, as it allows users to quickly find meaningful data. The classifier visualization functions as a keyword-based filter. The user can select pre-defined semantic filters, such as \textit{Safety} or \textit{Weather}, create their own filters, and intersect or union multiple filters according to their needs. Each filter contains an extensive list of associated keywords. When a filter is enabled, any data not containing a word from the filter is removed from the map. Importantly, the filtering mechanism affects all other visualizations, such as the temporal visuals and topic-modeling view, in that they will only be applied to the filtered data for more refined analysis. 

As discussed in the introduction, keyword-based matching is insufficient for finding relevant information as it can still result in filtered data that is semantically unrelated. This can considerably impede both the user experience and crisis prevention since users must still manually search through the filtered data to identify relevant data, such as requests for help during a natural disaster. 

\subsection{Interactive Learning}
Primarily motivated by SMART's imprecise filtering mechanism, our interactive learning approach improves real-time social media relevance classification by leveraging user feedback to identify and learn textual properties of relevant data. 

==> future_work.tex <==
\section{Future Work}

\subsection{Additional Visualizations}
Although SMART 2.0 provides integrated visuals and filtering and labeling interactions to quickly identify relevant tweets, additional high-level visualizations of relevant data can provide increased understanding of overall trends in the data. We plan to introduce another map layer, such as a heat map, to better understand geographical trends of relevant data. For instance, visually clustered groups of relevant data during a disaster event can alert the user to specific affected areas that might need attention or contain actionable information.

\subsection{Multi-user Support}
SMART 2.0 currently assumes all users share and train the same underlying models. However, it is possible that different users may wish to train the same models differently from other users, as the notion of relevancy ultimately depends on the individual. We plan to include user IDs with training requests so that they are associated with their models and can therefore train them independently. The scalability of multi-user support depends on the server architecture, as multiple users would send the server training and prediction data. Although we do not explicitly offer a solution in this paper, distributed servers, which share user model files, could process multiple user requests in a timely manner. 

\subsection{User-provided Relevant Data}
To accommodate time periods in which relevant data is scarce, we plan to introduce an interactive panel in which users can provide example tweets for specific relevance labels. As an example, if the user would like to train a \textit{Hurricane} classifier before a hurricane event, they could provide a relevant tweet such as ``I'm stuck in this hurricane. Please help!''. As such, the model may be able to detect relevant tweets once the hurricane begins as opposed to requiring user training during the event.

% Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.

% First and foremost, we still need to add several complementary visual features to the interface.
% For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.

% Second, the system currently only supports model training and prediction for one classifier and one user. 
% Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers.
% Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.

% Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model.
% Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. 
% By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.

% Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model.
% By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.

% Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.

==> implementation.tex <==


\section{Implementation}
    Our models were implemented with the \texttt{TensorFlow} ~\cite{tensorflow} and \texttt{Keras} ~\cite{keras} libraries. 
    % The model simulations were completed with an NVIDIA Quadro K4000 graphics card with 6874 MB memory.
    % The CNN implementation consists of the traditional convolutional and max-pooling layers before activation ~\cite{yin2017comparative}. We use Hochreiter's LSTM ~\cite{hochreiter1997long} and the traditional RNN ~\cite{elman1990finding} architectures as provided by \texttt{Keras}. 
    The selected CNN model interfaces with the SMART 2.0 web client through the \texttt{Django} ~\cite{django} framework.
    % Each user time the user labels ten tweets, they are transmitted to the server for model training. 
    % After the model is trained, all filtered tweets are sent back to the model again for prediction to synchronize user feedback with predicted relevance.

==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> test.tex <==
Social media data has been used extensively in a variety of applications, tools, and research endeavors due to its ability to provide useful information regarding people's thoughts, opinions, and behavior. For instance, social media data can be used to extract geographical movement patterns [4] and temporal distributions [33]. One particularly popular area is classifying social media into distinct groups, such as by sentiment [1, 5, 9, 10, 16, 19, 26, 27, 32] or certain topics [17]. 

However, traditional text classification techniques perform poorly since each social media message is short (e.g., 280 characters for Twitter), thereby providing insufficient contextual information. Not to mention, although considerable research has been conducted on natural language processing (NLP) classification tasks with various machine learning algorithms [1, 3, 5, 9, 10, 11, 14, 15, 16, 19, 20, 21, 26, 27, 28, 32], little attention has been directed towards the integration of user interaction with these machine learning models. We address these problems by specifically studying the topic classification engine in SMART, the Social Media Analytics and Reporting Toolkit [34] (Figure 1), and enhancing it with a long short-term memory (LSTM) neural network that utilizes the relatively new \textit{word2vec} model [15] for word embedding. 

SMART is an incredibly powerful tool that offers many features for analyzing social media data. SMART was primarily developed by researchers at Purdue University to provide situation awareness to law enforcement, government officials, and special interest groups. The system obtains social media posts from Twitter and Instagram in real-time and displays them on a map. The user is then able to apply a number of visualizations and filters to interactively examine and explore various data characteristics. For example, users can view the temporal distributions, topics, and most frequently used words of tweets, as well as enable visualization tools such as the heat map and content lens to view the map density and the top-used words within a certain area, respectively.

One considerably useful tool in SMART is its classifier visualization, which allows users to remove data unrelated to a specific topic through keyword matching. Specifically, each classifier contains a name, such as \textit{Security}, \textit{Weather}, or \textit{Job}, as well as a set of associated keywords. For instance, the \textit{Security} classifier might have the keywords \textit{shoot}, \textit{fire}, or \textit{steal} associated with it. If the user enables the \textit{Security} classifier, tweets that do not contain at least one of the classifier's pre-defined keywords are not included in the display. As such, SMART's classifier is incredibly useful for users who wish to only view data related to a certain category.

Nevertheless, SMART's classification scheme is not perfect since keyword matching fails to accurately capture semantic relevance. For example, if the user were to apply the \textit{Security} classifier, it would be possible for the tweets ``My house is on fire!'' and ``I was just fired from my job...'' to be displayed to the user since they both include the keyword \textit{fire}. However, the latter is unrelated to the intended semantic context of \textit{Security}. As such, SMART users are inconveniently tasked with further sorting through social media posts to find data related to what they meant for the classifier to capture. 

The first major goal of our work is to address this issue in SMART by introducing a machine learning model to learn tweet relevance. As a result, when a user applies a SMART classifier, the resulting data can be further classified according to relevance, thereby removing extraneous posts. However, since new user-defined classifiers can be added to SMART and irrelevant posts might still be incorrectly classified as relevant, it is important to allow the user to interactively correct erroneously labeled data. User feedback can help the model learn under which word contexts a tweet is relevant or not, thus improving predictive accuracy over time. Therefore, the second major goal of our work is to provide updated, interactive visuals to SMART's interface so that the user can more quickly and effectively find relevant data, as well as efficiently remove data that is not.

Overall, the major contributions of this paper are as follows:
\begin{itemize}
    \item A thoroughly tested neural network implementation using \textit{word2vec} for word embedding.
    \item A powerful user interface (UI) that allows users to interactively filter, analyze, and refine data according to relevance.
    \item A fully updated SMART application that dynamically retrieves tweet relevance and utilizes user feedback to train the model on the fly for increased predictive accuracy.
\end{itemize}

For the remainder of the paper, we discuss related work in section 2, the design and testing of our machine learning model in section 3, the implementation of the enhanced SMART UI in section 4, the results of the fully completed system in section 5, planned future work in section 6, and concluding remarks in section 7.

% An example of a floating figure using the graphicx package.
% Note that \label must occur AFTER (or within) \caption.
% For figures, \caption should occur after the \includegraphics.
% Note that IEEEtran v1.7 and later has special internal code that
% is designed to preserve the operation of \label within \caption
% even when the captionsoff option is in effect. However, because
% of issues like this, it may be the safest practice to put all your
% \label just after \caption rather than within \caption{}.
%
% Reminder: the "draftcls" or "draftclsnofoot", not "draft", class
% option should be used if it is desired that the figures are to be
% displayed while in draft mode.
%
%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
% where an .eps filename suffix will be assumed under latex, 
% and a .pdf suffix will be assumed for pdflatex; or what has been declared
% via \DeclareGraphicsExtensions.
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

% Note that the IEEE typically puts floats only at the top, even when this
% results in a large percentage of a column being occupied by floats.
% However, the Computer Society has been known to put floats at the bottom.


% An example of a double column floating figure using two subfigures.
% (The subfig.sty package must be loaded for this to work.)
% The subfigure \label commands are set within each subfloat command,
% and the \label for the overall figure must come after \caption.
% \hfil is used as a separator to get equal spacing.
% Watch out that the combined width of all the subfigures on a 
% line do not exceed the text width or a line break will occur.
%
%\begin{figure*}[!t]
%\centering
%\subfloat[Case I]{\includegraphics[width=2.5in]{box}%
%\label{fig_first_case}}
%\hfil
%\subfloat[Case II]{\includegraphics[width=2.5in]{box}%
%\label{fig_second_case}}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure*}
%
% Note that often IEEE papers with subfigures do not employ subfigure
% captions (using the optional argument to \subfloat[]), but instead will
% reference/describe all of them (a), (b), etc., within the main caption.
% Be aware that for subfig.sty to generate the (a), (b), etc., subfigure
% labels, the optional argument to \subfloat must be present. If a
% subcaption is not desired, just leave its contents blank,
% e.g., \subfloat[].


% An example of a floating table. Note that, for IEEE style tables, the
% \caption command should come BEFORE the table and, given that table
% captions serve much like titles, are usually capitalized except for words
% such as a, an, and, as, at, but, by, for, in, nor, of, on, or, the, to
% and up, which are usually not capitalized unless they are the first or
% last word of the caption. Table text will default to \footnotesize as
% the IEEE normally uses this smaller font for tables.
% The \label must come after \caption as always.
%
%\begin{table}[!t]
%% increase table row spacing, adjust to taste
%\renewcommand{\arraystretch}{1.3}
% if using array.sty, it might be a good idea to tweak the value of
% \extrarowheight as needed to properly center the text within the cells
%\caption{An Example of a Table}
%\label{table_example}
%\centering
%% Some packages, such as MDW tools, offer better commands for making tables
%% than the plain LaTeX2e tabular which is used here.
%\begin{tabular}{|c||c|}
%\hline
%One & Two\\
%\hline
%Three & Four\\
%\hline
%\end{tabular}
%\end{table}


% Note that the IEEE does not put floats in the very first column
% - or typically anywhere on the first page for that matter. Also,
% in-text middle ("here") positioning is typically not used, but it
% is allowed and encouraged for Computer Society conferences (but
% not Computer Society journals). Most IEEE journals/conferences use
% top floats exclusively. 
% Note that, LaTeX2e, unlike IEEE journals/conferences, places
% footnotes above bottom floats. This can be corrected via the
% \fnbelowfloat command of the stfloats package.

\section{Related Work}

\subsection{Sentiment Analysis and Classification}

% needed in second column of first page if using \IEEEpubid
%\IEEEpubidadjcol
	One of the most popular research areas in natural language processing is sentiment analysis and classification, especially as it relates to social media platforms such as Twitter [16]. Stanford researchers began the early analysis of Twitter sentiment [10]. Their approach consisted of using unigrams, bigrams, and parts-of-speech tags as features for learning keyword-based, naive bayes (NB), maximum entropy (ME), and support vector machine (SVM) sentiment classifiers. Several other unique approaches have also been taken. For instance, Gautam \textit{et al.} [9] used sentence adjectives as features in NB, ME, SVM, and WordNet models to learn sentiment; Paltoglou \textit{et al.} [19] took a lexicon-based method that specifically analyzed the text to predict sentiment (e.g., a negation term reverses the sentiment polarity of its neighboring word); Tang \textit{et al.} [27] sought to capture both sentiment and syntactic information by learning sentiment-specific word embeddings through neural networks; and Xiang \textit{et al.} [32] classified sentiment though a base-line SVM classifier with a robust feature set and a topic-based mixture model that separated tweets into topic groups which were then each classified with their own sentiment model. Innovative work was also carried out by Deng \textit{et al.} [5] in which Probabilistic Soft Models were used to analyze the sentiment of events and entities within texts. 
	
	However, the above research focuses on one aspect of our problem: sentiment. Although sentiment can differentiate tweets, it is not alone sufficient. For instance, tweets such as ``I was fired from my job'' and ``My house is on fire'' might be related in sentiment, but they are still semantically unrelated with regards to the word fire. This prompted us to explore \textit{word2vec} representations of twitter messages, which can inherently capture both sentiment and semantics by learning word context.
	
\subsection{Short Text Classification}
    Traditional text classification techniques perform poorly with short texts, such as social media messages, due to a lack of contextual information and low word frequencies. Nevertheless, numerous research endeavors have been made to improve such classification. For example, Chen \textit{et al.} [3] utilized external corpuses to derive multi-granular topics for short text feature enhancement; Hu \textit{et al.} [11] integrated semantic information from knowledge bases such as Wikipedia; and Phan \textit{et al.} [21] designed a framework to improve short text classification by constructing classifiers from large external datasets.
    
    In our work, we account for the shortness of social media messages by relying on external word embedding information from Google's \textit{word2vec} model [15], which was pre-trained on approximately 100 billion words from large text corpuses.

\subsection{Document Vectorization}
	Representing text documents as vectors (i.e., word embedding) has become increasingly popular since vectors can easily be used as feature inputs for machine learning models, such as clustering, to find semantic similarities. For example, Wong \textit{et al.} [30] represented search query documents as \textit{n}-dimensional vectors based on their topics and word associations. As a result, clustered documents could reveal related content.
	
	In specific, Google's \textit{word2vec} model has garnered attention in recent years due to its powerful ability to capture word sentiment and semantics [15]. One particularly interesting example is the work of Trieu \textit{et al.} [28], which used Twitter-based \textit{doc2vec} models (extensions of \textit{word2vec} models that indicate similarity between documents as opposed to words) and a modified clustering distance metric to classify news articles. The author's modified distance metric (which weighted not only the distance from \textit{q} to \textit{x}, but also the average distance of each of the \textit{K} nearest neighbors of \textit{q} to \textit{x}) could more easily detect semantic relevance between documents.
	
	Moreover, Abdelwahab \textit{et al.} [1] explored sentiment classification accuracies with a combination of \textit{word2vec}, \textit{doc2vec}, and other input features such as unigrams and bigrams. Additionally, Tang \textit{et al.} [26] used convolutional and gated recurrent neural networks to better account for semantic relationships among sentences within a document. One issue with the work of Abdelwahab \textit{et al.} [1] is that it averages the \textit{word2vec} vectors for input features, which removes syntactic information; \textit{doc2vec} also suffers from this. Although researchers have directly modified \textit{word2vec}'s skip-gram and continuous bag-of-word algorithms to preserve word order [14], there is no indication if semantic relationships between sentences are captured. Tang \textit{et al.} [26] sought to offer a direct solution to this. 
	
	Nonetheless, our approach differs in that we specifically use a LSTM neural network, which we found through experimentation to yield better results for our specific task, in combination with the \textit{word2vec} model. 
	
\subsection{Neural Networks and Machine Learning}
	Our research is heavily influenced by deep learning and machine learning, which have become particularly useful in classifying and clustering data. For instance, Kappeler \textit{et al.} [13] used deep neural networks to extract features from images, cluster the images according to feature similarities, and then train a classifier for each cluster to determine the image category (e.g., outdoors, man-made structure, etc.); Sharda \textit{et al.} [23] trained a neural network to predict movie box office performances based on relevant features such as the film rating (e.g., G, PG, etc.) and genre; and Pennacchiotti \textit{et al.} [20] employed a machine learning approach to predict Twitter users' political affiliation and ethnicity from inputs such as user tweeting behavior and their tweet content. Of course, our approach differs in that we are more interested in classifying social media data based on relevance, which requires a greater focus on NLP tasks, such as word embedding, as well as allowing the model to improve over time through direct user feedback. 
	
	Further, many traditional machine learning algorithms are conducted offline --- in other words, the models are trained on a static dataset. By contrast, online learning techniques, which can perform as well as offline techniques under certain circumstances [18], are used when the training data is supplied sequentially. Since data from SMART is interactively labeled by the user over time, online machine learning approaches are necessary. Specifically, we train on newly provided user-labeled data as well as recently used training samples to simulate offline learning in which batch data is used multiple times, thereby improving the model's performance (see section 3.3.2 for more details).

\subsection{Interaction}
	Although our work has deep roots in machine learning, the ultimate goal is to allow the user to interact with, filter, and sort tweets by semantic relevance, as well as mark incorrect labels. The model can then learn over time the most semantically-related tweets. This connects heavily to interactive machine learning, which has grown substantially over the past several years, producing innovative methods and allowing end-users to become more involved in the learning process [2, 7]. 
	Moreover, one particularly related example is the work of Dy \textit{et al.} [6], which allowed users to interactively select the desired subset of data features based on visualizing the corresponding clusters. Not to mention, Wall \textit{et al.} [29] introduced a novel visual analytics framework in which feature weights could be inferred from users' ranking of the data with Ranking SVM. 
	
	Our approach differs in that users will \textit{implicitly} rank the tweets by modifying the labels of the ones they find semantically unrelated and the ones they are more interested in or find more relevant. More specifically, a neural network can use the feature vectors as inputs and output an initial relevance ranking of the tweets. When the user adjusts the tweet labels, the network weights will change through backpropagation. As such, over time, tweets can be visually displayed and organized more closely to user preferences, thereby reducing the need to manually search for relevant tweets on the map.
	
\subsection{Machine Learning Visualization}
    Visualizations of machine learning algorithms and deep neural networks have been increasingly studied over the past years in an attempt to better understand their functionality. For instance, Kahng \textit{et al.} [12] developed the visual analytics system \textit{ActiVis} to interactively explore the components of large-scale deep neural networks through tightly integrated views, and Talbot \textit{et al.} [25] created the system \textit{EnsembleMatrix} that allows the user to build multiple classifier models and interactively view their confusion matrices. Further, Sacha \textit{et al.} [22] propsed a framework to discuss the various forms of human interaction with machine learning models in visual analytics systems and theorized that VA tools could increase knowledge and usability of machine learning components. 
    
    Nonetheless, these works focus on visualizing and interacting with machine learning models themselves to improve understanding. By contrast, we are interested in how interactive visuals can allow the user to efficiently improve a model's performance.
    
\subsection{Social Media Visualization}
    Visualization of social media data has also been extensively researched in an aim to better detect patterns and relationships between data samples. Chen \textit{et al.} [4] designed an immensely intriguing visual analytics system to analyze aggregated movement patterns among geo-tagged data to reveal social media users' behavior and visiting patterns. Additionally, Xia \textit{et al.} [31] developed \textit{CityBeat}, a powerful tool that analyzes streamed geo-tagged photos for extracting city events and trends, as well as detecting abnormalities in daily activities; Smith \textit{et al.} [24] also developed the \textit{NodeXL} tool to interactively visualize network structures of social media for determining a variety of data connections.
    
    Our work differs in that we are implementing social media visual tools specifically to interactively refine and view tweet relevance, with an emphasis on machine learning training.

\section{Machine Learning Model}
    
\subsection{Design}
    Google's \textit{word2vec} model [15] is able to excellently preserve semantic word relationships. The model is trained on roughly 100 billion words and represents each word as a 300-dimension vector. As such, \textit{word2vec} is a natural choice to embed words as vectors, which can then be used as inputs into a model for predicting relevance. As mentioned in the related work, many researchers have represented a sentence by converting each word to its vector, averaging the vectors, and then using the resulting feature vector for model training. However, averaging the vectors is not optimal since a sentence's syntactic information, which can inherently provide useful information about the sentence structure, is lost. To capture both semantic and syntactic information, we decided to represent a sentence as a matrix, where each row \textit{i} in the matrix is a 300-dimension vector  corresponding to word \textit{i} in the original sentence (Figure 2). 
    
    Furthermore, we used a neural network for learning tweet sentiment. The neural network takes as an input a tweet sentence matrix and outputs label probabilities. In specific, the network predicts the probability of a given tweet being (1) relevant, (2) not relevant, or (3) undecided, which can then be sent to the front end for user display.
    
    Overall, the high-level system workflow is illustrated in Figure 3. An incoming tweet is converted to a matrix consisting of \textit{word2vec} vectors and then sent to the neural network for classification. A label is assigned, and the tweet is displayed in the UI. If the user finds that it is labeled incorrectly, they can appropriately mark it to train the model for better prediction.

\subsection{Implementation}
    Since machine learning can be extremely complex, numerous libraries have been developed to support seamless, rapid implementation of various models and neural networks. We implemented our model in Python with the powerful \textit{keras} and \textit{tensorflow} libraries. The libraries provide well-defined APIs and considerable functionality for training and evaluating neural networks. 

\subsection{Testing}
    Due to the plethora of neural network types and parameter combinations, much of our efforts were devoted to finely tuning our model. Doing so allowed us to concretely determine the best model to solve our problem.

\subsubsection{Data Preparation}
    
    As with many classification tasks, it was necessary to obtain a dataset for training and testing. We used a public disaster-related tweet dataset provided by Figure Eight [8]. The dataset intuitively represents data that would result from applying a SMART classifier such as \textit{Disaster}. The dataset contains 10,876 tweets, each manually marked by contributors over time as (1) relevant, (2) not relevant, or (3) can't decide. 
    
    Of course, the data in its original form was not usable. To use it for model training, we applied \textit{regex} expressions to remove hashtags, unnecessary punctuation, hyperlinks, and symbols. We then converted the text to lowercase since capitalization is inconsistent among users and can lead to differences in word embedding, which is clearly undesirable. 
    
    After the text was cleaned, we converted each tweet into tokens and padded the token arrays to the maximum length of any token array in the dataset. This ensures equal length among the data. Each tokenized word in the tweet was then used as an index for the \textit{word2vec} model to retrieve its vector representation.

\subsubsection{Neural Network Experimentation}
    We first experimented with 3 well-known neural networks to determine which yielded the highest validation accuracy: a convolutional neural network (CNN); a simple recurrent neural network (RNN); and a long short-term memory (LSTM) neural network. 
    
    The experiment was relatively straightforward. We shuffled the first 7,000 tweets in the disaster dataset and used them for training the neural network. However, we wished to carry out our training in a way that could simulate user feedback. As such, we programmed a \textit{for} loop so that the NN would only train on 10 new tweets each iteration of the training cycle. This accurately simulates a user correcting the labels of 10 tweets and sending them to the server to train the model. The past 100 used tweet samples were also used for training so that the model could see the same data a few times for increased learning and predictive accuracy. Therefore, if the NN trained on data samples $train[100:200]$, the next iteration would train on samples $train[110:210]$. Next, we evaluated the model's performance on 900 separate tweets after each iteration to determine validation accuracy, which is the metric we wish to maximize.  
    
    We began by implementing a CNN with a basic 1-dimension convolution layer and 1-dimension max pooling layer. The output from these layers was then flattened and activated with a dense layer. The CNN testing results were quite good (Figure 4), but we still wished to test a few other neural networks.
    
    Next, we implemented a simple RNN, as provided by \textit{keras}. The RNN testing results were satisfactory (Figure 5), but could not compete with the CNN's.
    
    Our final neural network implementation was the LSTM neural network with a softmax activation function. The LSTM results (Figure 6) were superior to those for the CNN and RNN implementations.

    In the end, we selected the LSTM neural network for our model. The primary reason was that it yielded the highest validation accuracy ($81.66\%$) in our experiments. Nevertheless, another metric we strongly considered was the LSTM's number of iterations it required before achieving its average validation accuracy. Figure 6 demonstrates that approximately 20-30 iterations were needed for the model to achieve $81.66\%$ accuracy. Since each iteration adds 10 new tweets, 20-30 iterations corresponds to having trained on 200-300 tweets. As such, the user would have to mark 200-300 data samples to achieve that accuracy, which is a relatively reasonable number given that SMART displays thousands of tweets. Of course, we wish to minimize the number of manual user edits to avoid overburdening the user. However, the CNN and RNN took a comparatively larger number of iterations to reach their average validation accuracies, further supporting our decision to use the LSTM as our model.
    
    \subsubsection{Hyperparameter Tuning}
    
    After selecting the neural network, we robustly tuned the model hyperparameters. Initially, hyperparameter tuning proved to be a difficult task. We first attempted to test different hyperparameters through K-fold cross validation. However, the validation process had still not completed after a day, which was on only a handful of hyperparameter combinations out of thousands. As such, in order to more robustly tune our model, we decided to use the widely employed training-test data split scheme, as used in our neural network experimentation. Given that there were thousands of hyperparameter combinations, we automated the task with \textit{talos}, a Python library specifically equipped to tune any \textit{keras} model. Since the automation process was unable to use our training scheme in the neural networks experiment (i.e., training on 10 new incoming tweets each iteration), we defined a static training and testing set. The former consisted of 2,800 randomly shuffled samples, and the latter consisted of 1,200 samples. 
    The automation process was executed on the Purdue ITaP clusters with 2,400 different hyperparameter combinations and completed after approximately 4 days.

    Needless to say, we were quite pleased with the results (Figure 7), as the highest accuracy achieved --- $88.06\%$ --- was comfortably higher than the $81.66\%$ accuracy from the base LSTM we had tested on. However, many of the hyperparameters are impractical since we were unable to simulate 10 new incoming tweets each iteration. For instance, training the model on 200 epochs can take 5-10 minutes, and a $3.07\%$ learning rate can yield loss errors when the number of epochs or training size are small. With multiple users and the need for reasonably timed training on a small number of labeled tweets from the user, we decided to use some of the optimal hyperparameters, such as the activation, loss, and dropout parameters, in combination with others we had previously used. We further tested a set of these parameter combinations and gathered their validation accuracies (Figure 8).

     The results from Figure 8 illustrate that the highest validation accuracy improved on our original LSTM model yet again. However, we found the graph of the highest validation accuracy parameter set to be revealing (Figure 9). Compared to our original LSTM neural network (Figure 6), the average validation accuracy was achieved after a much greater number of iterations. Specifically, our original LSTM neural network was able to achieve at least an 80 accuracy after approximately 20-30 iterations, which corresponds to 200-300 training samples. By contrast, the model in Figure 9 took at least 50 iterations --- 500 training samples --- to achieve a $75\%-80\%$ accuracy and did not even reach its $84.72\%$ accuracy until approximately 80-90 iterations --- 800-900 training samples. In fact, all models from Figure 8 took at least 20-30 iterations longer than our base LSTM to achieve an $80\%$ accuracy. As discussed previously, in the context of interactive machine learning, we wish to reduce the number of samples the user has to provide before achieving an acceptable accuracy. 

	 All in all, based on the hyperparameter tuning results, we decided to use our original LSTM implementation since it had an acceptable accuracy --- $81.66\%$ --- and required significantly less training to achieve this accuracy than the other models.

\subsection{\textit{Django} Server}
    
    Since Python is well-equipped with powerful libraries for machine learning tasks, we sought to keep our LSTM model implementation in Python rather than implementing it in another language to communicate with SMART's front end. We decided to use \textit{Django}, a popular web applicaton framework that supports Python back end development. Not to mention, given that our model might be used by other systems than SMART, \textit{Django} could serve that purpose since it allows the model to essentially function as a self-contained API in that any client can make simple, well-defined calls to the server endpoints to retrieve information or execute a set of commands (e.g., train the model). 
    
    Our current implementation of the \textit{Django} server has three major endpoints. The first one is $/init/$, which creates a new model and saves its state to a $.h5$ file on the server. The second endpoint is $/getLabels/$. When a client makes a request to the server at this endpoint, it must also supply an array of tweets. The server then embeds the tweets as vectors using \textit{word2vec}, predicts the label probabilities for each tweet, and returns the labels and associated probabilities as an array to the client for further analysis. The final endpoint is $/updateLabels/$. When a client makes a request to this endpoint, it must also provide both an array of tweets and corresponding array of labels. The server then trains the model on the provided data, saves its updated state, and returns a success status.

\section{User Interface}
    The next major component of our work was the implementation of the enhanced SMART UI. Given that SMART is a complex system and that we needed a simple interface to test and modify the \textit{Django} server with, we first developed a prototype front end and implemented a variety of new capabilities. After verifying correct functionality, we integrated our prototype's interface with SMART and made several additional augmentations for improved interactivity and visualization of relevance metrics.

\subsection{Prototype Implementation}
    As with SMART's front end, we coded the prototype front end in JavaScript (Figure 10). Rather than streaming tweets in real-time, we decided to simply read in the labeled disaster tweet \textit{.csv} file we had used for the neural network training and display it in a table, with the text and associated relevance label as columns. Since the prototype contained no classifiers, we assumed the disaster data could represent data that had been pre-filtered (i.e., the user had applied a classifier as in SMART to begin viewing semantically-related data). Furthermore, the front end also consisted of a background map with the tweets as individual dots (which we randomly assigned); the user could click on a dot to reveal a tweet's text.

    The first primary interactive tool we added was allowing the user to filter the table by relevance. To accomplish this, we added a drop down box at the top of the relevance column. The user could click on the drop down to select the 'All' (default), 'Only Relevant', or 'Only Not Relevant'' option. As the names suggest, selecting the respective drop down option would display all tweets in the table regardless of relevance, only tweets with a 'Relevant' label, or only tweets with a 'Not Relevant' label.

    Moreover, we also allowed the user to specifically click on a 'Relevant' or 'Not Relevant' label to change it to 'Not Relevant' or 'Relevant', respectively (essentially a toggle). This allowed the user to relabel incorrectly classified data.
    
    Further, when a tweet's label was altered by the user from its original label, the tweet's row would be highlighted in light brown to indicate that it had been changed. For example, in Figure 10, the first two rows indicate that the user changed their labels to 'Not Relevant'. Importantly, the 'Not Relevant' rows that are not highlighted indicate that their labels have not been adjusted by the user. This helps better distinguish user-labeled 'Not Relevant' tweets from unmodified 'Not Relevant' labeled tweets.

    Finally, the user could click the 'Save' icon at the top left corner of the table to save the highlighted rows with their new labels. Doing so removed the highlight and simulated sending the modified tweets and their new labels to the model for training.
    
    Although the prototype allowed us to concretely implement our initial design concepts and ideas, it lacked many features, prompting our transition to integrating with SMART and adding several additional components. For example, the prototype interface did not allow the user to directly relabel a tweet's relevance from its map point; users were unable to view a table entry's corresponding map location; and filtering the table by relevance was not reflected on the map. Development in SMART allowed us to easily add these features, as many were already provided by the system.


\subsection{SMART Implementation}
\subsubsection{Table}
    
    As in the UI prototype, enhancing the table was our first major focus (Figure 11). However, unlike our prototype, which read data from a \textit{.csv} file with pre-defined relevance labels, SMART retrieves data in real-time and stores the tweets in a database provided by the \textit{TaffyDB} JavaScript library. As such, to retrieve the necessary relevance data, we added a relevance field to the database. As a result, when the tweets are obtained for table display, their relevance fields are also extracted.
    
    Furthermore, the user can click directly on relevance labels to change them. However, the labels are not restricted to only 'Relevant' and 'Not Relevant', but also include a 'Can't Decide' label for tweets that are not definitively relevant or irrelevant, but might be one or the other depending on certain circumstances. As in the prototype, a drop down box is also included. It allows the user to specifically filter the table down to only tweets with 'Relevant', 'Not Relevant', or 'Can't Decide' labels.
    
    A major addition to the geo-message table is the visual display of a tweet's \textit{degree} of relevance. In specific, the probabilities of a tweet being 'Relevant', 'Not Relevant', or 'Can't Decide' are represented as a horizontal segmented bar graph and sized proportional to their respective percentages. We chose light blue, red, and gray colors for the bar segments and corresponding relevance labels since they blend in nicely with the geo-message table and SMART color designs. Naturally, the tweet's exact relevance label corresponds to the maximum of the 3 probabilities. For example, if the probability of a tweet being relevant is $50\%$, the not relevant probability is $30\%$, and the undecided probability is $20\%$, the tweet will be assigned the label 'Relevant'.

    Additionally, the user can also hover over a specific probability class (Figure 12) --- 'Relevant', 'Not Relevant', or 'Can't Decide' --- and click on it to sort tweets by that probability. Specifically, clicking on a probability class first sorts the tweets by that probability in \textit{decreasing} order (i.e., largest probabilities at the top of the table). If the same probability class is clicked a second time, the tweets are then arranged by the probability in increasing order (i.e., smallest probabilities at the top of the table). A third click on the same probability class returns the tweets to their default arrangement --- sorting by date in decreasing order. For example, clicking on the 'Relevant' probability class the first time sorts the tweets by decreasing relevance (Figure 13).
    
    Finally, since retrieving tweet relevance labels from the server can take a few seconds, we used a spin  animation to replace the relevance label and probability columns so that the user can intuitively infer that data is being retrieved (Figure 14).
    
\subsubsection{Map}
    
    The next major UI enhancement was adding a relevance label to map point pop-ups (Figure 15), which was relatively straightforward to implement, as SMART's map layer --- \textit{OpenLayers} --- allows HTML embedding in marker pop-ups. Since a tweet map point's \textit{longitude} and \textit{latitude} coordinates are extracted from the \textit{TaffyDB} database, we modified the code to also extract the relevance label and display that in the pop-up in addition to a tweet's time and text. Although not indicated in Figure 15, the user is able to click on the colored relevance label to change it to any of the 3 relevance labels, which will be immediately reflected in the geo-message table. Therefore, if the user finds a tweet on the map that they believe is incorrectly labeled, they can label it directly as opposed to having to search for it in the geo-message table. 

    Additionally, if the user selects a filter such as 'Only Relevant' from the drop down box in the table, the map view is also filtered along with the table. Consequently, the tweets on the map will always match those displayed in the geo-message table. 

\subsubsection{Server Communication}
    SMART communicates with the \textit{Django} server by first making an AJAX call to the web server with the necessary data in POST fields. The web server then executes the \textit{RelevanceManager.php} file to directly contact the \textit{Django} server. Any information is then ultimately returned back to the browser for processing and updates. Informal timings indicate that requests from SMART for relevance labels or model training take only 5-10 seconds at most, which is excellent.
    
\subsubsection{Dataflow}
    
    When the user selects a SMART classifier, all of the tweets that pass the classifier are sent to the server to retrieve their predicted relevance labels.
    
    Furthermore, we refined exactly \textit{when} user-modified labels are sent to the server for model training. Unlike the prototype, tweets with user-modified labels are not highlighted in light brown, and users are not able to click on a 'Save' icon to send modified tweets to the server for training. We updated this process to make the user experience more enjoyable. Rather, when a user changes a label, it is essentially added to a queue. To prevent server bombardment, relabeled data is only sent after the user has marked 10 unique tweets. After the relabeled data is sent and the model is trained, all classified tweets are then sent back to the model for another round of prediction since the user's updated labels could have changed the labels of other unmodified data.

\section{Results}
    In order to determine the system's efficacy, we carried out a preliminary use case. We analyzed a large region in California and applied the \textit{Security} classifier. Given the recent wildfire in California, we hoped to find many relevant tweets that could be used for training. After relabeling only 20 tweets, we saw a noticeable adjustment in tweet relevance classification. In specific, Figure 16 demonstrates the predicted labels of new incoming tweets after we had trained the model. We were delighted to notice many correct classifications. For example, the bottom 2 posts relating to an earthquake and fire were properly classified. However, some of the tweets were not properly labeled. For instance, the ``San Francisco Fire Dept. is on the ground assisting with the heroic firefighting effort...'' tweet should be marked as ``Relevant''.
    
    Nonetheless, given that the model was only trained on 20 samples, the results are extremely promising and indicate that relevance classification responds to user feedback. 

\section{Future Work}
    Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.

\section{Conclusion}
    In this paper, we provided a unique approach to classifying social media relevance. In specific, we detailed the implementation, testing, and fine-tuning of our neural network model. Additionally, we discussed the extensive visual updates we applied to the SMART system, which allow users to interactively filter, refine, view, and examine tweets based on their categorized relevance. Finally, we described the completed system's capabilities and dataflow in which users are able to directly modify tweet labels for continual model training and improvement. Although the system has several future improvements underway, our preliminary case study yielded promising results and verified proper functionality.
    
        Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.
        Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.
        Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.
        Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.
    
        Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.
    
        Although the updated SMART system functions considerably well, there are a vast number of improvements and additions we plan to make in the coming weeks.
    
    First and foremost, we still need to add several complementary visual features to the interface. For example, a dotted line underneath the relevance labels would more clearly indicate to the user that they can click on it, and providing buttons on the map pop-ups might be more intuitive and visually appealing for a user to change a tweet's relevance.
    
    Second, the system currently only supports model training and prediction for one classifier and one user. Since SMART is a multi-user platform --- with multiple classifiers representing different semantic contexts ---, it is necessary for each user to be able to train each of their own classifiers. Fortunately, this task is relatively straightforward since we can pass additional fields to the \textit{Django} server, such as \textit{userID} and \textit{classifierID}, to indicate which model should be used on the data.
    
    Third, it is extremely important to add an interactive panel in which users can enter example tweets for specific relevance labels, which can then be used to train the model. Since a large majority of tweet data can be irrelevant for certain classifiers, training the model with only irrelevant data can prevent it from correctly classifying data that should be labeled relevant. By allowing the user to provide specific examples, such as ``I am going to bomb my school'' as a relevant instance for the \textit{Security} classifier, the model can more quickly delineate the classification boundary between what is relevant and what is not, thereby improving predictive accuracy.
    
    Fourth, several tweets contain slang or informal language, as well as emotes, which are currently overlooked in our model. By converting slang and emotes to full words and correcting any misspellings, the model could more accurately account for a tweet's semantic meaning, yielding better prediction.
    
    Fifth, although we carried out an initial case study, we still need to further test on different classifiers and events, as well as perhaps obtain input from SMART users on the usability and effectiveness of the enhanced application.

